Training neural mapping schemes for satellite altimetry with simulation data

Satellite altimetry combined with data assimilation and optimal interpolation schemes have deeply renewed our ability to monitor sea surface dynamics. Recently, deep learning (DL) schemes have emerged as appealing solutions to address space-time interpolation problems. The scarcity of real altimetry dataset, in terms of space-time coverage of the sea surface, however impedes the training of state-of-the-art neural schemes on real-world case-studies. Here, we leverage both simulations of ocean dynamics and satellite altimeters to train simulation-based neural mapping schemes for the sea surface height and demonstrate their performance for real altimetry datasets. We analyze further how the ocean simulation dataset used during the training phase impacts this performance. This experimental analysis covers both the resolution from eddy-present configurations to eddy-rich ones, forced simulations vs. reanalyses using data assimilation and tide-free vs. tide-resolving simulations. Our benchmarking framework focuses on a Gulf Stream region for a realistic 5-altimeter constellation using NEMO ocean simulations and 4DVarNet mapping schemes. All simulation-based 4DVarNets outperform the operational observation-driven and reanalysis products, namely DUACS and GLORYS. The more realistic the ocean simulation dataset used during the training phase, the better the mapping. The best 4DVarNet mapping was trained from an eddy-rich and tide-free simulation datasets. It improves the resolved longitudinal scale from 151 kilometers for DUACS and 241 kilometers for GLORYS to 98 kilometers and reduces the root mean squared error (RMSE) by 23% and 61%. These results open research avenues for new synergies between ocean modelling and ocean observation using learning-based approaches.

==> tables/benchmark.tex <==
\begin{table}[h!]
\begin{tabular}{ll||llll|rrr|}
\toprule
 && SSH  & Deep  & Calibrated on & Physical  & RMSE & nRMSE  & $\lambda_x$ \\
 &&  Only &  Learning & &  Model &  (cm) &  () &  (km) \\
\midrule
(a) & 4DVarNet &  Yes & Yes & Simulation data & None & 5.9  & 0.91  & 98 \\
(b) & MUSTI & No &  Yes & Satellite data & None & 6.3  & 0.90  & 112 \\
(c) & ConvLstm-SST & No &  Yes & Satellite data & None & 6.7  & 0.90  & 108 \\
(d) & ConvLstm &  Yes &  Yes & Satellite data & None & 7.2  & 0.89  & 113 \\
(e) & DYMOST&  Yes & No & Satellite data & QG & 6.7  & 0.90  & 131 \\
(f) & MIOST &  Yes & No & Satellite data & None & 6.8  & 0.90  & 135 \\
(g) & BFN-QG &  Yes & No & Satellite data & QG & 7.6  & 0.89  & 122 \\
(h) & DUACS &  Yes & No & Satellite data & None & 7.7  & 0.88  & 151 \\
(i) & GLORYS12 & No & No & Satellite data & NEMO & 15.1  & 0.77  & 241 \\
\bottomrule
\end{tabular}
\caption{Benchmarks of different methods. (b) \cite{Archambault_Filoche_Charantonnis_Béréziat_2023}, (c and d)\cite{Martin_Manucharyan_Klein_2023}, (e)\cite{Ballarotta_Ubelmann_Rogé_Fournier_Faugère_Dibarboure_Morrow_Picot_2020}, (f)\cite{Ubelmann_Dibarboure_Gaultier_Ponte_Ardhuin_Ballarotta_Faugère_2021}, (g)\cite{Guillou_Metref_Cosme_Ubelmann_Ballarotta_Sommer_Verron_2021}, (h)\cite{Taburet_Sanchez-Roman_Ballarotta_Pujol_Legeais_Fournier_Faugere_Dibarboure_2019}, (i)\cite{Jean_Michel_Eric_Romain_Gilles_Angélique_Marie_Clément_Mathieu_Olivier_Charly_et_al._2021}  }
\label{tab:bench}
\end{table}

==> tables/data.tex <==
\begin{table}[h!]
    \centering
\begin{tabular}{l||cccc|}
\toprule
{} & Resolution & Reanalysis & Tide & DAC  \\
\midrule
NATL60\cite{Ajayi_Le_Sommer_Chassignet_Molines_Xu_Albert_Cosme_2020}               &      1/60 $^\circ$ &               No &            No &                   No  \\
eNATL60-t\cite{Brodeau_Sommer_Albert_2020}         &      1/60 $^\circ$ &               No &           Yes &                  Yes  \\
eNATL60-0\cite{Brodeau_Sommer_Albert_2020}         &      1/60 $^\circ$ &               No &            No &                  Yes  \\
GLORYS12-r\cite{Jean_Michel_Eric_Romain_Gilles_Angélique_Marie_Clément_Mathieu_Olivier_Charly_et_al._2021} &      1/12 $^\circ$ &              Yes &            No &                   No  \\
GLORYS12-f\cite{Jean_Michel_Eric_Romain_Gilles_Angélique_Marie_Clément_Mathieu_Olivier_Charly_et_al._2021}   &      1/12 $^\circ$ &               No &            No &                   No  \\
ORCA025 \cite{Bernard_Madec_Penduff_Molines_Treguier_Le_Sommer_Beckmann_Biastoch_Böning_Dengg_et_al._2006}             &       1/4 $^\circ$ &               No &            No &                   No  \\
\bottomrule
\end{tabular}
\caption{Summary table of the synthetic data tested for training}
\label{tab:data}
\end{table}

==> tables/results.tex <==
\begin{table}[h!]
\begin{tabular}{l||rrrr|}
\toprule
Training Data & RMSE (cm) & nRMSE () & nRMSE$_{sla}$ () & $\lambda_x$ (km) \\
\midrule
NATL60 & 5.9  & 0.91  & 0.80  & 98 \\
eNATL60-t & 5.9  & 0.91  & 0.80  & 100 \\
eNATL60-0 & 5.9  & 0.91  & 0.80  & 100 \\
GLORYS12-r & 6.3  & 0.90  & 0.78  & 106 \\
GLORYS12-f & 6.7  & 0.90  & 0.77  & 119 \\
ORCA025 & 7.1  & 0.89  & 0.76  & 126 \\
\bottomrule
\end{tabular}
\label{tab:res}
\caption{Performance comparison of 4dVarNet mapping schemes trained on different simulated datasets. The first column show the source of the training dataset as described in \ref{tab:data}. The subsequent columns shows }
\end{table}
